Variable-Shot Adaptation for Online Meta-Learning

Few-shot meta-learning methods consider the problem of learning new tasks from a small, fixed number of examples, by meta-learning across static data from a set of previous tasks. However, in many real world settings, it is more natural to view the problem as one of minimizing the total amount of supervision --- both the number of examples needed to learn a new task and the amount of data needed for meta-learning. Such a formulation can be studied in a sequential learning setting, where tasks are presented in sequence. When studying meta-learning in this online setting, a critical question arises: can meta-learning improve over the sample complexity and regret of standard empirical risk minimization methods, when considering both meta-training and adaptation together? The answer is particularly non-obvious for meta-learning algorithms with complex bi-level optimizations that may demand large amounts of meta-training data. To answer this question, we extend previous meta-learning algorithms to handle the variable-shot settings that naturally arise in sequential learning: from many-shot learning at the start, to zero-shot learning towards the end. On sequential learning problems, we find that meta-learning solves the full task set with fewer overall labels and achieves greater cumulative performance, compared to standard supervised methods. These results suggest that meta-learning is an important ingredient for building learning systems that continuously learn and improve over a sequence of problems.

==> Online Variable-Shot Meta-Learning arxiv/defs.tex <==
%% editing comment
\newcommand{\cmt}[1]{{\footnotesize\textcolor{red}{#1}}}
\newcommand{\note}[1]{\cmt{Note: #1}}
\newcommand{\todo}[1]{\cmt{To-Do: #1}}


%% abbreviations
\newcommand{\x}{\mathbf{x}}
\newcommand{\z}{\mathbf{z}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\w}{\mathbf{w}}
\newcommand{\data}{\mathcal{D}}

\newcommand{\etal}{{et~al.}\ }
\newcommand{\eg}{e.g.\ }
\newcommand{\ie}{i.e.\ }
\newcommand{\nth}{\text{th}}
\newcommand{\pr}{^\prime}
\newcommand{\tr}{^\mathrm{T}}
\newcommand{\inv}{^{-1}}
\newcommand{\pinv}{^{\dagger}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\gauss}{\mathcal{N}}
\newcommand{\norm}[1]{\left|#1\right|}
\newcommand{\trace}{\text{tr}}

%% specifics for the paper
\newcommand{\reward}{r}
\newcommand{\policy}{\pi}
\newcommand{\mdp}{\mathcal{M}}
\newcommand{\states}{\mathcal{S}}
\newcommand{\actions}{\mathcal{A}}
\newcommand{\observations}{\mathcal{O}}
\newcommand{\transitions}{\mathcal{T}}
\newcommand{\initial}{\mathcal{I}}
\newcommand{\horizon}{H}
\newcommand{\rewardevent}{R}
\newcommand{\probr}{p_\rewardevent}
\newcommand{\metareward}{\bar{\reward}}

\newcommand{\pihi}{\pi^{\text{hi}}}
\newcommand{\pilo}{\pi^{\text{lo}}}
\newcommand{\ah}{\mathbf{w}}

\newcommand{\loss}{\mathcal{L}}
\newcommand{\eye}{\mathbf{I}}

\newcommand{\model}{\hat{p}}

\newcommand{\pimix}{\pi_{\text{mix}}}

\newcommand{\pib}{\bar{\pi}}
\newcommand{\epspi}{\epsilon_{\pi}}
\newcommand{\epsmodel}{\epsilon_{m}}

\newcommand{\upd}{\mathcal{U}}

\newcommand{\ind}{\delta}

%% math
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\en}{\mathcal{E}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\ot}{\bo_t}
\newcommand{\st}{\bs_t}
\newcommand{\at}{\ba_t}
\newcommand{\op}{\mathcal{O}}
\newcommand{\opt}{\op_t}
\newcommand{\kl}{D_\text{KL}}
\newcommand{\tv}{D_\text{TV}}
\newcommand{\ent}{\mathcal{H}}

\newcommand{\bzhi}{\bz^\text{hi}}

==> Online Variable-Shot Meta-Learning arxiv/experiments.tex <==
%
\section{Experiments}
%
\label{sec:experiments}

Our experiments aim to address the following questions, in both offline and online problem settings. In the more standard offline meta-learning setting, we aim to answer: \textbf{(1)} How does our variable-shot meta-learning method compare to prior methods, when evaluated with variable shots\rebuttal{ in the offline setting}? \textbf{(2)} Does our theoretically motivated learning rate rule match the performance of learning per-shot learning rates? We then integrate our variable-shot method into the online setting, to study: \textbf{(3)} Does variable-shot learning improve the regret in the \rebuttal{online} incremental meta-learning setting? \textbf{(4)} Does our \rebuttal{online} incremental meta-learning algorithm attain better cumulative regret than standard empirical risk minimization?
%
%
Details regarding the architecture of the models and the training setup are presented in Appendix~\ref{app:offline_details}. 

\iclr{While our method can accommodate any standard meta-learning problem, we intentionally focus our evaluation on meta-learning problems with \emph{non-exclusive} tasks, since this setting is particularly relevant in the online setting, which we will discuss in the subsection below and since this setting known to be especially difficult~\citep{yin2019meta}. With non-exclusive tasks, it is technically possible for the model to learn to solve all tasks in zero shot, which provides for a fair comparison to non-meta-learning online methods, such as the ``follow the learder'' method that trains on all data seen so far (indicated as ``TOE'' in Section~\ref{sec:online_exp}). However, in order to attain the best possible regret, an effective meta-trained model must still learn to adapt, so as to solve new tasks quickly \emph{before} it has learned to solve all tasks in zero shot. Standard meta-learning methods often perform poorly in this regime, due to a memorization problem~\citep{yin2019meta}, where they learn to only solve the meta-training tasks in zero shot, failing to either solve or adapt to the new task. We use three non-mutually exclusive datasets for our offline and online meta-learning experiments respectively and one mutually-exclusive dataset for the offline setting only, which are listed as follows:}\\
\iclr{\textbf{(1) Rainbow MNIST (non-mutually exclusive).}} Based on the MNIST digit recognition dataset, this dataset~\citep{ftml} consists of digits transformed in different ways: 7 backgrounds with different colors, 2 scales (half and original size), and 4 rotations of 90 degree intervals, which leads to 56 total tasks in combination. Each task contains 900 images applied with one of the transformation listed above (See Appendix~\ref{app:offline_details} for visualization); \textbf{(2) Contextual MiniImagenet (non-mutually exclusive).}
This dataset, adapted from MiniImagenet~\citep{ravi2016optimization}, is meant to provided a non-mutually-exclusive variant of the MiniImagenet few-shot recognition task, such that non-meta-learning baselines can feasibly solve this task. We use the same images and classes as MiniImagenet, but formulate each class as a separate binary classification problem. The model receives two images as input: a reference image that determines the current task, and a query image, and the goal is to output a binary label indicating whether the query image belongs to the same class as the reference image, or not. \iclr{In this case, each class in the MiniImagenet constitutes a task, which makes the task space large and the problem challenging.} We include a visualization of the architecture for solving this dataset in Figure~\ref{fig:arch} in Appendix~\ref{app:miniimagenet_details};
%
%
%
%
%
\textbf{(3) Pose Prediction (non-mutually exclusive).} Following \cite{ftml} and \cite{yin2019meta}, we construct a multi-task dataset with $65$ tasks based on the Pascal 3D data~\citep{xiang2014beyond} where each task corresponds to a different object with a random camera angle. We render the image each object using MuJoCo~\citep{mujoco} with a random orientation. We only use this dataset in the online setting;
\textbf{(4) Omniglot (mutually exclusive).} This dataset~\citep{omniglot} has 20 instances of 1623 characters from 50 different alphabets where each instance is drawn by a different person. We only use this dataset in the offline setting and include the results in Appendix~\ref{app:offline_exclusive}.
%
%
%
%

\subsection{Offline Meta-Learning Experiments}
\label{sec:offline_exp}

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\begin{table*}[t]
\centering
\scriptsize
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{ lccccc  }
 \toprule
 %
    Dataset & Method & 0-Shot & 1-Shot & 10-Shot & 20-Shot \\
 \midrule
    \multirow{3}{*}{Rainbow MNIST} & MANN~\citep{mann} & $66.41 \pm 1.55$ & $66.49 \pm 1.68$ & $67.09 \pm 1.38$ & $66.95 \pm 1.12$ \\
    & MAML~\citep{maml} & $71.30 \pm 0.53$ & $71.13 \pm 0.91$ & $74.78 \pm 1.12$ & $\mathbf{78.67} \pm 0.68$\\
    & MAML-VL (ours) & $\mathbf{73.14} \pm 0.65$ & $\mathbf{73.45} \pm 0.61$ & $\mathbf{74.87} \pm 0.38$ & $76.59 \pm 0.36$ \\
    & MAML-VS (ours) & $72.72 \pm 0.45$ & $72.91 \pm 0.15$ & $73.89 \pm 0.60$ & $77.17 \pm 0.10$\\
    \hline
    \multirow{3}{*}{Contextual MiniImagenet} & MANN~\citep{mann} & $\mathbf{64.85} \pm 0.04$ & $\mathbf{64.90} \pm 0.19$ & $64.78 \pm 0.63$ & $65.50 \pm 0.50$\\
    & MAML~\citep{maml} & $61.36 \pm 0.48$ & $56.80 \pm 0.65$ & $63.82 \pm 0.09$ & $63.84 \pm 0.31$ \\
    & MAML-VL (ours) & $61.17 \pm 1.95$ & $59.11 \pm 3.06$ & $\mathbf{66.09} \pm 2.93$ & $66.15 \pm 4.74$ \\
    & MAML-VS (ours) & $63.37 \pm 0.71$ & $63.19 \pm 1.14$ & $65.89 \pm 0.10$ & $\mathbf{66.94} \pm 0.14$ \\
 \bottomrule

\end{tabular}
\end{adjustbox}
\vspace{-0.2cm}
\caption{\small \rebuttal{\textbf{Complete Results for Offline Rainbow MNIST and Offline Contextual MiniImagenet.} Comparison of MAML, MANN, MAML-VL (ours) and MAML-VS (ours). The results are classification accuracies averaged over 3 random seeds, $\pm$ one standard deviation. On Rainbow MNIST, MAML-VL (ours), that learns a learning rate per shot, does better in 0, 1, and 10-shot setting, which is the most effective in this relatively simple digit classification task. MAML-VS (ours) achieves comparable performance in all four settings in this experiment. On Contextual MiniImagenet, which is a challenging image classification problem with large task space, MAML-VS (ours) achieves better performance in 20-shot classification accuracies while maintaining competitive performances in 0, 1 and 10-shot settings. Overall, MAML-VS achieves the best or comparable performances in all 8 settings, which indicates that our theoretically-motivated inner learning rate scaling rule would excel in the online setting, which is empirically shown in Table~\ref{tbl:online_final}.}}
\label{tbl:offline_app}
\vspace{-0.2cm}
\end{table*}

We first evaluate our variable-shot methods, MAML-VS and MAML-VL, in the offline setting, in comparison to MAML~\citep{maml} and MANN~\citep{mann}, which uses a non-gradient based recurrent meta-learner. \rebuttal{The offline experiments mainly serve as a unit test for our variable-shot learning rate rule, whereas the online incremental experiments illustrate the setting we are most interested in, and where variable-shot learning is practically important.} Experiment setup details, including descriptions of baselines, the dataset setup, and model architectures can be found in Appendix \ref{app:offline_details}. \rebuttal{Note that, as discussed in Section~\ref{sec:rw}, non-parametric meta-learning methods require at least one shot for each class, making them inapplicable to non-mutually exclusive tasks where the total number of support datapoints is often much lower than the total number of classes. Hence, we cannot evaluate these prior methods in this setting. However, we adapt the non-parametric meta-learning methods to online settings by reusing data from past tasks when the total number of support datapoints is less than the number of classes, which we will discuss in Section~\ref{sec:online_exp}.}
%
As shown in Table \ref{tbl:offline_app},
%
\rebuttal{our method, MAML-VL, achieves the best performance in 5 out of the 8 settings in both datasets, while MAML-VS achieves the best performance in the 20-shot classification accuracy on Contextual MiniImagenet, which is a challenging problem with a large task space, and attains comparable performance in the 7 other settings.}
In both experiments, training for variable shot with a single learning rate (MAML) causes the algorithm to sacrifice
%
0-shot and 1-shot performance in favor of better performance with more shots (10 and 20). In the Contextual MiniImagenet setting especially, 1-shot performance is \emph{significantly} lower than even the 0-shot performance. For MANN, variable shot training instead biases the model toward good 0-shot and 1-shot performance, and sacrifices performance with more shots. We expect both issues to be problematic in the online setting: good few-shot performance is important in the later stages of training, where each task can be mastered with just a few samples, and good many-shot performance is critical for difficult tasks or early on in training. Our methods, MAML-VS\rebuttal{ and MAML-VL}, perform well with all numbers of shots, and performance improves as more examples are observed.


%

%

%

\subsection{Online Incremental Meta-Learning Experiments}
\label{sec:online_exp}

\begin{table*}[t]
\scriptsize
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{ lccc  }
 \toprule
 %
    Method & Incremental Rainbow MNIST & Incremental Contextual MiniImagenet & Incremental Pose Prediction \\
 \midrule
    TOE~\citep{ftml} & $16516.6\pm172.5$ & $2314.5\pm363$ & $125.2\pm0.6$\\
 \hline
    FTML~\citep{ftml} & $4804.2\pm302.8$ & $1037.7\pm116.1$ & $135.5\pm18.8$\\
 \hline
    \rebuttal{FTML+Meta-SGD~\citep{li2017meta}} & \rebuttal{$4699.0 \pm 212.0$} & \rebuttal{$1027.3 \pm 35.8$} & \rebuttal{$125.0 \pm 9.4$}\\
 \hline
    FTML-VL (ours) & $4502.7\pm477.0$ & $1033.9\pm21.5$ & $141.3\pm30.3$\\
 \hline
    FTML-VS (ours) & $\mathbf{4484.7}\pm133.8$ & $\mathbf{1020.0}\pm40.8$ & $\mathbf{119.1}\pm3.2$\\
 \bottomrule
\end{tabular}}
%
\vspace{-5pt}
\caption{\footnotesize 
%
Final cumulative regret on Incremental Rainbow MNIST, Incremental Contextual MiniImagenet and Incremental Pose Prediction. Results are cumulative regrets averaged over 3 random seeds, $\pm$ one standard deviation. FTML-VS outperforms other methods in all three domains.}
%
\label{tbl:online_final}
\vspace{-0.6cm}
\end{table*}

\begin{table*}[t]
\scriptsize
\centering
\begin{tabular}{ lcc  }
 \toprule
 %
    \rebuttal{Dataset} & \rebuttal{A-GEM~\citep{chaudhry2018efficient}} & \rebuttal{FTML-VS (ours)} \\
 \midrule
    \rebuttal{Incremental Rainbow MNIST} & \rebuttal{$14292.19 \pm 201.72$} & \rebuttal{$4484.70 \pm 113.83$}\\
 \bottomrule
\end{tabular}
\vspace{-5pt}
\caption{\footnotesize 
%
\rebuttal{Comparison between A-GEM~\citep{chaudhry2018efficient} and FTML-VS on Incremental Rainbow MNIST. Results are cumulative regrets averaged over 3 random seeds, $\pm$ one standard deviation. FTML-VS achieves superior results compared to A-GEM.}}
\label{tbl:agem}
\vspace{-0.2cm}
\end{table*}


\begin{table*}[t]
\scriptsize
\centering
\begin{tabular}{ lcc  }
 \toprule
 %
    \rebuttal{Dataset} & \rebuttal{Incremental ProtoNet~\citep{snell2017prototypical}} & \rebuttal{FTML-VS (ours)} \\
 \midrule
    \rebuttal{Incremental Rainbow MNIST} & \rebuttal{$34812.7 \pm 6197.7$} & \rebuttal{$19207.7 \pm 282.4$}\\
 \bottomrule
\end{tabular}
\vspace{-5pt}
\caption{\footnotesize 
%
\rebuttal{Comparison between Incremental ProtoNet~\citep{snell2017prototypical} and FTML-VS on Incremental Rainbow MNIST with adapted data-generating scheme discussed in Section~\ref{sec:online_exp}. Results are cumulative regrets averaged over 3 random seeds, $\pm$ one standard deviation. FTML-VS significantly outperforms Incremental ProtoNet.}}
\label{tbl:protonet}
\vspace{-0.5cm}
\end{table*}

To answer questions \textbf{(3)} and \textbf{(4)}, we evaluate FTML-VS in the online incremental setting. To evaluate the performance of our approach, we compare our FTML-VS to: \iclr{(1) \textbf{Train on everything (TOE)~\citep{ftml}}, which is the standard empirical risk minimization approach that trains a single predictive model on all the data available so far, i.e. $\{\hat{D}_i\}_{i=1}^t$. The trained model is directly tested on $\data^\text{test}_t$ without any adaptation; (2) \textbf{FTML~\citep{ftml}}, which trains an online meta-learner with fixed inner learning rate and is evaluated on the adaptation performance on $\data^\text{test}_t$; (3) \textbf{FTML-VL (Ours)}, which trains an online meta-learner with a learned inner learning rate for each number of shots ranging from $0$ to $M$; \rebuttal{(4) \textbf{FTML+Meta-SGD~\citep{li2017meta}}, which learns per-parameter learning rates for FTML; (5) \textbf{Incremental ProtoNet~\citep{snell2017prototypical}}, which adapts \cite{snell2017prototypical}, one of the most widely used non-parametric meta-learning method to the online incremental meta-learning setting; (6) \textbf{A-GEM~\citep{chaudhry2018efficient}}, which is a popular continual learning algorithm that prevents catastropic forgetting.}}
%
%
%
%
%
%
%
%
%

For \textbf{Incremental Rainbow MNIST}, we set the proficiency threshold $C$ at $85\%$ classification accuracy \iclr{computed on a minibatch of test data $\data_t^\text{test} \subset \data_t$ where $\data_t^\text{test} \cap \hat{D}_t(s) = \emptyset$ for each task $t$}, and move on to the next task when this threshold is crossed or after $2000$ steps. For \textbf{Incremental Contextual MiniImagenet}, we set the proficiency threshold $C$ at $75\%$ classification accuracy \iclr{computed on $\data_t^\text{test}$}. For \textbf{Incremental Pose Prediction}, we consider mean-square error as the metric and do not advance the task automatically. We discuss the details of the online procedure of each dataset in Appendix~\ref{app:online_details}. We evaluate the performance based on the final cumulative regret \iclr{$\regret$, which is computed by accumulating the test losses on $\data_t^\text{test}$ during evaluation time for each task $t$}, as shown in Table~\ref{tbl:online_final} and include the regret curves over the \rebuttal{online} incremental meta-learning process of all methods in all domains in Appendix~\ref{app:online_details}. \rebuttal{We also include additional ablation studies in Appendix~\ref{app:online_ablation}.}

According to Table~\ref{tbl:online_final}, in all three domains, FTML-VS attains smallest regret after training all the tasks sequentially compared to other methods, suggesting the importance of using our learning rate rule in the \rebuttal{online} incremental meta-learning setting \iclr{with non-mutually exclusive datasets}. Moreover, FTML-VS outperforms TOE by a large margin, which indicates that our online meta-learning method is able to solve tasks more efficiently than empirical risk minimization by leveraging the shared task structure to quickly adapt to each new task. \rebuttal{Finally, FTML-VS also achieves lower final cumulative regret than FTML + Meta-SGD, suggesting that our theoretically sound rule of selecting learning rates for different number shots is more effective than simply learning different learning rates for each parameter. It is also worth noting that learning per-parameter learning rates is complementary to our method and can be combined to further improve performances. We leave this for future work.}
%
%

%
%
\rebuttal{As discussed in Section~\ref{sec:rw}, continual learning methods also tackle the problem of learning a stream of tasks but rather focus on minimizing negative transfer and do not maintain a buffer of the past data, which our method does. For completeness of the comparison, we compare FTML-VS to a widely used continual learning method, A-GEM, on the Incremental Rainbow MNIST dataset with the same online procedure described above. As shown in Table~\ref{tbl:agem}, FTML-VS achieves much better cumulative regret compared to A-GEM. This result is unsurprising, as prior continual learning works focus primarily on minimizing negative backward transfer and compute considerations, as opposed to our goal of accelerating forward transfer through meta-learning.}
%
%

%
%
\rebuttal{Finally, non-parametric meta-learning methods~\citep{snell2017prototypical, allen2019variadic, cao2020a} can naturally work well in with different number of shots, making them an important point of comparison. However, as noted in Section~\ref{sec:rw} and Section~\ref{sec:offline_exp}, they are not indirectly applicable to settings where the number of shots is smaller than the number of classes. Therefore, to provide a proper comparison,
we adapt prototypical networks~\citep{snell2017prototypical} to our online incremental setting in the following manner:
%
%
when we do not have the support datapoints for a particular class in the current task, we compute the prototype of this class by sampling data of this class from previous tasks. We call the adapted prototypical networks as Incremental ProtoNet. We compare FTML-VS to Incremental ProtoNet following the above data-generating protocol and the same online procedure as in the Incremental Rainbow MNIST experiment described in the paragraph above. As shown in Table~\ref{tbl:protonet}, FTML-VS outperforms Incremental ProtoNet by a significant margin, suggesting that our theoretically motivated learning rate selection rule is pivotal in the \rebuttal{online} incremental meta-learning setting compared to non-parametric meta-learning methods, which require the minimum number of shots to be greater than or equal to the number of classes.}

==> Online Variable-Shot Meta-Learning arxiv/intro.tex <==
\section{Introduction}
\label{sec:intro}

Standard machine learning methods typically consider a static training set, with a discrete training phase and test phase. However, in the real world, this process is almost always cyclical: machine learning systems might be improved with the acquisition of new data, repurposed for new tasks via finetuning, or might simply need to be adjusted to suit the needs of a changing, non-stationary world. Indeed, the real world is arguably so complex that, for all practical purposes, learning is never truly finished, and any real system in open-world settings will need to improve and finetune perpetually~\citep{chen2017machine,youtube_recs}. 
In this continual learning process, meta-learning provides the appealing prospect of accelerating how quickly new tasks can be acquired using past experience, which in principle should make the learning system more and more efficient over the course of its lifetime. However, current meta-learning methods are typically concerned with asymptotic few-shot performance~\citep{maml,snell2017prototypical}. For a continual learning system of this sort, we instead need a method that can minimize both the number of examples per task, and the number of tasks needed to accelerate the learning process.

Few-shot meta-learning algorithms aim to learn the structure that underlies data coming from a set of related tasks, and use this structure to learn new tasks with only a few datapoints. While these algorithms enable efficient learning for new tasks at test time, it is not clear if these efficiency gains persist in online learning settings, where the efficiency of both meta-training and few-shot adaptation is critical. Indeed, simply training a model on all received data, \iclr{i.e., standard supervised learning with empirical risk minimization,} is a strong competitor \iclr{since supervised learning methods are known to generalize well to in-distribution tasks in a zero-shot manner. Moreover,} it's not clear that meta-learning algorithms can improve over such methods by leveraging shared task structure \iclr{in online learning settings}.
%
%
%
%
Provided that it is possible for a single model to fully master all of the tasks with enough data, both meta-learning and standard empirical risk minimization approaches should produce a model of equal competence. However, the key hypothesis of this work is that meta-learned models will become more accurate more quickly in the middle of the online learning process, while data is still being collected, resulting in lower overall regret in realistic problem settings.

%
%
\begin{figure}
\centering
\vspace{-0.2cm}
\small
\includegraphics[width=0.78\textwidth]{figures/teaser.png}
\vspace{-0.2cm}
\caption{\footnotesize \textbf{\rebuttal{Online} incremental meta-learning.} We visualize our \rebuttal{online} incremental meta-learning problem setting in the above figure using the Incremental Pose Prediction dataset discussed in Section~\ref{sec:experiments}. At round t, the current task is to predict the pose of a sofa with a small training set containing several datapoints of the sofa with different orientations. After one epoch of training, we evaluate the few-shot generalization performance on a test datapoint where the number of shots equals the size the task's training set. If the test performance exceeds some proficiency threshold C, we advance to the next task, i.e. predicting the pose of the airplane. Otherwise, we add another training example of the sofa to the training set and repeat the above process.
}
\vspace{-0.7cm}
\label{fig:teaser}
\normalsize
\end{figure}
\iclr{To study this hypothesis}, we consider a practical online learning problem setting, \iclr{which we refer to as online incremental learning}, where the algorithm must learn a sequence of tasks, and datapoints from each task are received sequentially. Once a model reaches a certain level of proficiency, the algorithm may move on to training the model on the next task. \iclr{This problem is crucial to solve in the real world, especially in settings where online data collection and supervision signals are costly to obtain. One example} of such a problem definition is a setting where a company receives requests for object classifiers, sequentially at different points in time. Data collection and labels are expensive, and the company wants to spend the least amount of money on acquiring a good classifier for each request.
%
%
%
%
%
%
%
%
%
%
%
%
A \iclr{major challenge for meta-learning} that arises in this problem setting is \iclr{to design a meta-learning algorithm that can adapt with variable shots}: As data from new tasks is incrementally introduced, at any given point in time, the model may have access to zero, a few, or many datapoints for a provided task. \iclr{The goal of this work is to achieve variable-shot adaptation while minimizing the total required amount of supervision in terms of number of shots needed to master each new task. The desired \rebuttal{online} incremental meta-learning algorithm is expected to generalize to a new task with decreasing numbers of shots over the course of training. We illustrate our problem setting in Figure~\ref{fig:teaser}.}
%
%

%

The key contributions of this work are (a) a new meta-learning algorithm that can adapt
%
%
to variable amounts of data, and (b) an online version of this algorithm that addresses the above problem setting \iclr{of online incremental learning}. We theoretically derive our \iclr{variable-shot meta-learning algorithm}
%
%
and combine it with deep neural networks for effective online learning on challenging sequential problem settings.
We find that our approach can outperform empirical risk minimization and \iclr{a previous online meta-learning method~\citep{ftml}}
%
%
on two online image classification problems consisting of sequences of classification tasks and one online regression problem.
%
%


%

==> Online Variable-Shot Meta-Learning arxiv/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}
\usepackage{amsthm, amssymb, bbm}
\usepackage{thm-restate}
\usepackage{thmtools}
\usepackage{mathtools}

% Math
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{corollary}{Corollary}
\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{notation}{Notation}
\newtheorem{obs}{Observation}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\newcommand{\update}{\mathbf{U}}
\newcommand{\regret}{\text{Regret}_T}

==> Online Variable-Shot Meta-Learning arxiv/method.tex <==
\newcommand{\updatev}{\mathbf{U}^\text{V}}
%
\newcommand{\var}{\text{Var}}
\newcommand{\buffer}{\mathcal{B}}


\section{The \rebuttal{Online} Incremental Meta-Learning Problem Statement}

%

%

%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


%
The \rebuttal{online} incremental meta-learning problem statement extends the online meta-learning setting~\citep{ftml}, where the tasks arrive one at a time. In our proposed incremental setting, the data \emph{within} each task also arrives one data point at a time, and the goal of the model is to minimize the cumulative regret summed over all of the tasks. A model that can adapt to a new task more quickly in fewer shots should attain lower regret. A model that can do so \emph{while having seen as few previous tasks as possible} will be even better. Formally, the learning process is divided into ``tasks'' and ``shots''. Each time step, the learner either receives one more ``shot'' (data point) for the current task, or transitions to a new task and receives the first shot for that task. \rebuttal{In practice, instead of generating 1 datapoint every time step, the learner receives a small batch of datapoints every few time steps.} Let $t$ denote the current task counter, and $s$ the current shot counter. At each step $s$ for task $t$, the model has access to $\hat{\data}_t(s)$, the dataset for the current task, which presently contains $s$ shots. The model can adapt to the current task using $\hat{\data}_t(s)$, and must then attain the lowest possible risk on that task.

To realize this setting, we extend the update procedure defined in Section~\ref{sec:prelim} to the variable-shot setting, formally $\update_t(\theta_t, \alpha, s)$. The risk in round $t$ with $s$ shots in this incremental setting is defined as $f_t(\update_t(\theta_t,\alpha, \min\{s, M\}))$ where $M$ is some large scalar \iclr{representing the maximum number of shots per task.}
%
%
%
%
The risk defined above suggests that the performance of the model is only evaluated using the $s$-shot risk $f_t(\update_t(\theta_t,\alpha, s))$, when there are $s <= M$ datapoints in the current datasets, \iclr{and always use $M$-shot risk when there are more than $M$ datapoints.}
%
%
%
%

%
%
\iclr{Now that we have defined our measure of incremental risk, we will discuss when the model can transition from one task to the next. Intuitively}, we want the model to be able to ``complete'' a task and transition to a new task as soon as it has achieved a requisite accuracy on that task. For instance, in the example in Section~\ref{sec:intro} of the company that receives requests for object classifiers, the company might choose to stop collecting training data for a given task once accuracy on that task is good enough, and move on to the next customer. We formalize this by introducing a threshold value $C$, such that when $f_t(\update_t(\theta_t,\alpha, s)) \leq C$ at step $s$, the learner switches to the next task immediately. In this way, a very efficient model that can adapt and master a task in just a few data points will attain lower overall regret \iclr{and solve the full sequence of tasks with fewer overall datapoints,}
%
%
since it will need fewer shots for each task.
%
%

To summarize, the overall \rebuttal{online} incremental meta-learning process looks like this:
%
%
%
%
%
%
%
%
\textbf{(1)} At the start of round $t$, the meta-learner selects a model parameterized by parameter $\theta_t$;
\textbf{(2)} The world chooses a task $\task_t \sim p(\task)$;
\textbf{(3)} At each step $s = 0, \dots$, the dataset $\hat{\data}_t(s)$ receives one datapoint;
\textbf{(4)} At step $s = 0, \dots$, the model updates $\theta_t$ as $\theta'_t = \update_t(\theta_t,\alpha, s)$;
\textbf{(5)} At step $s = 0, \dots$, the model is evaluated with $f_t(\update_t(\theta_t,\alpha, s))$ \iclr{and if $f_t(\update_t(\theta_t,\alpha, s)) \leq C$, the agent will advance}
%
%
 to the next round. When the advancement happens, denote $S_t = s$.
The objective of incremental meta-learning is to minimize the regret over all the rounds, \rebuttal{resembling the objective of online learning~\citep{Hannan,Kalai2005EfficientAF}, which we state} as follows:
\vspace{-0.05in}
\begin{align}
    \regret &= \sum_{t=1}^T\sum_{s=0}^{S_t}f_t(\update_t(\theta_t,\alpha, \min\{s, M\}))\nonumber -\min_\theta\sum_{t=1}^T\sum_{s=0}^{S_t}f_t(\update_t(\theta,\alpha, \min\{s, M\})),
\end{align}
%
%
where $\{\theta_t\}_{t=1}^T$ is a sequence of models at round $t = 1, \dots, T$. Similar to FTML, we aim to obtain a meta-learner that learns each task in the data-incremental setting, while attaining minimal regret.

\section{Variable-Shot Model-Agnostic Meta-Learning}
\label{sec:maml_vs}
%

The first step toward designing an \rebuttal{online} incremental meta-learning algorithm that can address this problem statement is to design a method that can handle variable numbers of shots, since in the incremental setting, the model will need to accommodate settings ranging from zero-shot at the beginning of each task to many-shot at the end. Attaining the lowest regret therefore depends crucially on maximally utilizing whatever task data may be available. We will therefore first design a variable-shot generalization of MAML in the standard \emph{offline} setting, and then apply it to the \emph{online} setting to provide a viable approach for \rebuttal{online} incremental meta-learning.
%

%
\subsection{A Na\"{i}ve Solution}

A naive solution would simply involve applying MAML with varying numbers of datapoints used to compute the inner graduate updates. During meta-training, the number of datapoints could be drawn uniformly from $\{0, \dots, M\}$ for some $M \in \mathbb{Z}^+$. The corresponding meta-training objective is then given as $\min_{\theta}\frac{1}{N}\sum_{i=1}^N \mathbb{E}_{s \sim \text{Unif}(0,M)}\left[f_i(\theta-\alpha \nabla_{\theta}\hat{f}^s_i(\theta))\right]$.
%
%
%

Unfortunately, as we will see in Section~\ref{sec:experiments}, this approach does not perform well when the number of shots varies, since the adaptation process is not aware of the number of shots that are available. Intuitively, when more data is available, the model should be able to deviate further from the prior parameter vector $\theta$, since the larger dataset provides us with more information about the task. Mathematically, this can be captured by the variance of the inner gradient. The variance of the inner gradient depends on $s$ as follows: $\var(\nabla_{\theta}\hat{f}^s_i\!(\theta)) = \var\left(\nabla_\theta\frac{1}{s}\sum_{j=1}^s\ell(\mathbf{h}(\mathbf{x}_j;\theta), \mathbf{y}_j)\right) = \frac{1}{s}\var(\nabla_\theta\ell(\mathbf{h}(\mathbf{x};\theta), \mathbf{y}))$
%
%
%
%
%
%
where the last equality follows from the property of the variance of the sum of i.i.d. random variables. The above equation indicates that the inner gradient variance inversely scales with the number of shots, but the model is unaware of this fact, since it is only updated via the average gradient. Therefore, the model has no way to know that it should ``trust'' the gradient more when more shots are available, leading to poor performance in the variable shot setting. This is also shown empirically in Section~\ref{sec:offline_exp}.

\subsection{The Learning Rate Scaling Method}
\label{sec:scaling}


Intuitively, if we have a lower variance gradient, we can take larger steps along that gradient. Therefore, a natural way to vary the model update based on the number of datapoints is to change the inner learning rate. It is well known in standard supervised learning that the optimal learning rate scales with batch size \citep{l.2018a}. One way to incorporate this observation into a variable-shot MAML algorithm would be to meta-learn \emph{different} learning rates for each number of shots. As we will see in Section~\ref{sec:offline_exp}, this approach, which we call MAML-VL \rebuttal{(variable-shot and learning)}, can indeed improve over standard MAML. However, this requires meta-learning an additional parameter for every possible number of shots, which can become impractical as the maximum number of shots increases. 

Instead, we can derive a simple rule for the optimal learning, which we will show can work even \emph{better} than meta-learning separate rates for each number of shots. First, let us define $\update_t(\theta, \alpha) = \theta - \alpha\nabla_\theta f_t(\theta)$ to be the ideal update rule given the average gradient. We can view this as the update rule for the limiting case of infinite shots, since $\update_t(\theta, \alpha) = \lim_{s \rightarrow \infty} \update_t(\theta, \alpha, s)$ in distribution by the law of large numbers. Let $\beta^*$ be the optimal learning rate such that $\update_t(\theta, \beta^*)$ attains optimal performance, i.e. $\beta^* = \arg\min_{\beta} \mathbb{E}_{\task_t}\left[f_t(\update_t(\theta, \beta))\right]$.
%
%
This can be interpreted as the optimal inner learning rate when $s \rightarrow \infty$. We want to find an \iclr{optimal $s$-shot learning rate $\alpha^*_{s}$} that imitates this behavior for a finite $s$. Specifically, we solve for the value of $\alpha^*_{s}$ that minimizes the mean square error between the adapted parameters: $\alpha^*_{s} = \arg\min_{\alpha} \mathbb{E}_{\task_t}\left[ ||\update_t(\theta, \alpha, s) - \update_t(\theta, \beta^*)||_2^2 \right]$.
%
%
%

\begin{theorem}
The optimal learning rate for the $s$-shot case is
$\alpha^*_s = \left(1 - \frac{1}{1 + \frac{C_2}{C_1}s}\right) \beta^*$,
where \mbox{$C_1 =   \mathbb{E}_{\task_t} \left[  \var( \nabla_\theta\ell(\mathbf{h}(\mathbf{x};\theta), \mathbf{y}) ) \right] \nonumber$} and  \mbox{$C_2 = \mathbb{E}_{\task_t} \left [||\mathbb{E}_{\data_t}\nabla_\theta\ell(\mathbf{h}(\mathbf{x};\theta), \mathbf{y})||_2^2\right]$}.
%
%
%
%
%
%
\label{thm:learning_rate}
\end{theorem}

We provide the proof in Appendix \ref{app:proof}. 
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
The quantities $C_1$, $C_2$ and $\beta^*$ are all functions of the parameters $\theta$, and thus require re-estimation each time we update $\theta$ during meta-training. In practice, we denote $\beta \coloneqq \beta^*$ as the learned learning rate and $\eta \coloneqq \frac{C_2}{C_1}$ as the learned scaling factor, and treat them as parameters that are meta-learned jointly with $\theta$. Denote $\alpha_s(\beta,\eta) = \left(1 - \frac{1}{1 + \eta s}\right) \beta$ as the learnable scaled learning rate with parameters $\beta$ and $\eta$.
%
In contrast to MAML-VL, which must meta-learn a number of learning rates that scales with the maximum number of shots, here we only meta-learn two additional scalar-valued parameters.
This leads to our proposed model-agnostic meta-learning with variable-shot and scaling (MAML-VS) algorithm, whose meta-training objective is given below:
\vspace{-0.03in}
\begin{align}
    \min_{\theta, \beta, \eta}\frac{1}{N}\!\sum_{i=1}^N\!\mathbb{E}_{s \sim \text{Unif}(0,M)}\!\left[f_i(\theta-\alpha_s(\beta, \eta) \nabla_{\theta}\hat{f}^s_i(\theta))\right]\!.
\end{align}

%

\section{Online Incremental Meta-Learning with Variable-Shot MAML}
%

With MAML-VS defined in the section above, we are ready to present the algorithm for the \rebuttal{online} incremental meta-learning setting. In following two subsections, we will discuss an online incremental meta-learning algorithm capable of variable-shot generalizations (Section~\ref{sec:ftml_vs}) and its practical instantiation (Section~\ref{sec:practical_algs}).


%
\subsection{Follow the Meta-Leader with Variable-Shot and Scaling}
\label{sec:ftml_vs}
We extend FTML~\citep{ftml} to the \rebuttal{online} incremental meta-learning setting by enabling the meta-learner to handle variable-shot data with the scaling rule in MAML-VS.
%
%
Specifically, in \iclr{the \rebuttal{online} incremental meta-learning setting}, the model parameter $\theta$ and the scaled learning rate $\alpha_s(\beta, \eta)$ defined in Section~\ref{sec:scaling} are updated in the following way:
\vspace{-0.05in}
\begin{align}
    \!\theta_{t+1}, \beta, \eta=\argmin_{\theta, \beta, \eta}\!\sum_{j=1}^t\sum_{s=0}^{S_j}f_j(\update_j(\rebuttal{\theta}, \alpha_s(\beta, \eta), s))\label{eq:ftml_vs}.
\end{align}
\iclr{We term our \rebuttal{online} incremental meta-learning algorithm FTML-VS.} Intuitively, for the current round $t+1$, FTML-VS plays the best variable-shot meta-learner in hindsight after each round based on all the meta-learned models attained in previous rounds $j=1\dots t$. In practice, we of course cannot calculate the exact loss $f_j$, and therefore must approximate it using stochastic gradient descent methods, which will be presented in the next subsection.


\subsection{FTML-VS in Practice}
\label{sec:practical_algs}

Optimizing Equation~\ref{eq:ftml_vs} is not feasible in practice as it has no closed form solution. We only have access to a portion of $\task_t$ in round $t$, and thus the population risk $f_t$ is impossible to compute exactly, as discussed by~\citet{ftml}. We adopt online stochastic gradient descent algorithms to resolve these issues. At step $s$ in round $t$, we compute gradients of our model parameters $\theta_t$ and scale learning rate $\alpha_K(\beta, \eta)$ where $K$ is the number of shots sampled in a minibatch using the following procedure:
\vspace{-0.15in}
\begin{enumerate}
    \itemsep0em
    \item Draw a task $\task_j: j\sim\kappa(t)$ (or a minibatch of tasks) uniformly from the set of tasks the agent has seen so far $\{\task_i\}_{i=1}^t$, where $\kappa(t)$ is the uniform distribution on $\{1,\dots, t\}$. Let $\hat{\data}_j = \hat{\data}_j(s)$ if \rebuttal{$j = t$} and otherwise $\hat{\data}_j = \hat{\data}_j(S_j)$, which are all the data accumulated for task $\task_j$ in the previous round.
    \item Sample $K \sim \nu(j)$, where $\nu(j)$ is uniformly distributed on $\{0,\dots, M(j)\}$ with $M(j) = \min\{M, |\hat{\data}_j|\}$.
    \item Sample a minibatch $\data_j^\text{tr} \subset \hat{\data}_t(s)$ of size $K$ to compute the inner gradient updates using the derived scaled learning rate $\alpha_K(\beta, \eta)$.
    \item Sample another minibatch $\data_j^\text{val} \subset \hat{\data}_t(s)$ to compute the gradients $\mathbf{g}^{\theta_t}, \mathbf{g}^{\beta}, \mathbf{g}^{\eta}$ for updating the model parameter $\theta_t$ along with parameters of scaled learning rate, $\beta$ and $\eta$ respectively.\label{eq:practical_ftmlvs_update}
    \vspace{-0.1cm}
\end{enumerate}
%
%
where \iclr{we denote $J = \mathbb{E}_{j \sim \kappa(t), K \sim \nu(j)}\left[\loss(\data_j^\text{val}, \update_t(\theta_t, \alpha_K(\beta, \eta), K))\right]$, $\update_t(\theta_t, \alpha, K)\!=\!\theta_t - \alpha_K(\beta, \eta)\nabla_{\theta_t}(\loss(\data_t^\text{tr}, \theta_t))$ and $\mathbf{g}^\theta = \nabla_{\theta_t} J$, $\mathbf{g}^{\beta} = \nabla_{\beta} J$ and $\mathbf{g}^{\eta} = \nabla_{\eta} J$.}
Note that in the case of zero-shot adaptation, i.e. $K=0$, $\update_t(\theta_t, \alpha_K(\beta, \eta), K)$ \iclr{corresponds to the parameter at the previous round, i.e. $\theta_{t-1}$. }
%



%

%
%

%



%
\iclr{We outline the complete algorithm in Algorithm~\ref{alg:mamlincremental} in Appendix \ref{app:algo} with some implementation details in Appendix \ref{app:impl_detail}. The algorithm learns $\theta$, $\beta$, and $\eta$. 
%
%
We also include the training procedure and the evaluation protocol in Appendix~\ref{app:algo}.}
%

%
%
%
%

%

%



==> Online Variable-Shot Meta-Learning arxiv/prelim.tex <==
%
%
\newcommand{\task}{\mathcal{T}}

\section{Preliminaries}
\label{sec:prelim}

Meta-learning algorithms optimize for efficient adaptation to new tasks. To define the meta-learning problem, let $p(\task)$ denote a \emph{task distribution}, where each task $\task_i \sim p(\task)$ consists of a dataset \rebuttal{$\data_i \coloneqq \{\mathbf{x}, \mathbf{y}\}$} with i.i.d. input and output pairs. If we have a predictive model $\mathbf{h}(\mathbf{x};\theta)$ with some parameter $\theta$ and a loss function $\ell$, such as the cross entropy between the predicted label distribution and the true label distribution in a classification problem, the risk of $\task_i$, $f_i$, can be computed as \rebuttal{$f_i(\theta) = \mathbb{E}_{(\mathbf{x}, \mathbf{y})\sim\data_i}\left[\ell(\mathbf{h}(\mathbf{x};\theta), \mathbf{y})\right].$} At meta-training time, $N$ tasks $\{\task_i\}_{i=1}^N$ are sampled from $p(\task)$ and meta-learning algorithms \iclr{aim to learn how to quickly learn these tasks}
%
%
such that, at meta-test time, the population risk $f_j(\theta)$ of the unseen tasks $\task_j \sim p(\task)$ is minimized quickly.

In this work, we build on the model-agnostic meta-learning (MAML) algorithm~\citep{maml}. 
MAML achieves fast adaptation to new tasks by optimizing a set of initial parameters $\theta_\text{MAML}$ that can be quickly adapted to the meta-training tasks $\{\task_i\}_{i=1}^N$. Thus, at meta-test time, after a small number of gradient steps on $\theta_\text{MAML}$ with $K$ datapoints from $\data_j$, the model can minimize $f_j$ for the new task $\task_j$. 
%
%
Note that $K$ is a small and fixed number across all tasks. Formally, MAML achieves such an initialization by optimizing the following objective: \iclr{$\min_{\theta_\text{MAML}} \frac{1}{N} \sum_{i=1}^N f_i(\update_i(\theta_\text{MAML}, \alpha, K_i))$}
%
%
%
%
%
%
where $\alpha$ is the inner gradient step size, \iclr{$\update_i(\theta, \alpha, K_i) = \theta - \alpha \nabla_{\theta}\hat{f}^K_i(\theta)$ denotes the gradient update in the inner loop for task $i$, and }$\hat{f}^K_i(\theta) = \frac{1}{K}\sum_{j=1}^K\ell(\mathbf{h}(\mathbf{x}_j;\theta), \mathbf{y}_j)$ is the empirical risk of $\task_i$ based on a minibatch with $K$ datapoints sampled from $\data_i$. Hence, MAML can be viewed as optimizing for K-shot generalization.
%
%

In the online setting, prior work~\citep{ftml} has proposed the follow-the-meta-leader (FTML) algorithm, which adapts MAML to an online meta-learning setting where the meta-learner learns to adapt to tasks that arrive in a sequence. In this online meta-learning setting, the meta-learner faces a sequence of loss functions $\{\ell_t\}_{t=1}^\infty$ in each round $t$, where each of the tasks \iclr{share some common structure that could be captured by the meta-learner.}
%
%
The goal of the meta-learner is to find a sequence of models parametrized by $\{\theta_t\}_{t=1}^\infty$ that performs well on the sequence of loss functions after making some task-specific update procedures $\update_t(\theta_t, \alpha, K): \theta_t \in \Theta, K\in\mathbb{N} \rightarrow \theta' \in \Theta$ where $K$ is a fixed number of datapoints used to perform the update. In FTML, which adapts MAML to the online setting,  $\update_t(\theta_t, \alpha, K)$, \iclr{as defined in the paragraph above, is the inner gradient update w.r.t. the empirical risk with $K$-shot data $\hat{f}^K_t$ at round $t$.}
%
%
%
The performance of FTML is typically measured using the regret that compares the sum of population risks to the cumulative population risks with some fixed model parameter computed in hindsight: $\regret = \sum_{t=1}^Tf_t(\update_t(\theta_t, \alpha, K))-\min_\theta\sum_{t=1}^Tf_t(\update_t(\theta, \alpha, K))$.
%
%
%
%
Analogously to the standard follow-the-leader (FTL) algorithm~\citep{Hannan,Kalai2005EfficientAF}, FTML optimizes $\theta_t$ as \rebuttal{$\theta_{t+1} = \argmin_\theta\sum_{j=1}^tf_j(\update_j(\theta,\alpha, K))$}.
%
%
%
As mentioned above, the number of datapoints used for computing updates, $K$, is always fixed in both offline and online meta-learning settings. However, in the sequential learning setting, where datapoints for each task arrive incrementally, the model is required to handle varying numbers of datapoints from different tasks, and hence needs to generalize to new tasks quickly using \emph{any} amount of data. Our method is designed to tackle this problem setting, which we will discuss in the next section.


==> Online Variable-Shot Meta-Learning arxiv/related_work.tex <==
\section{Related Work}
\label{sec:rw}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

Prior work in meta-learning has studied how to acquire learning rules~\citep{schmidhuber1987,bengiobengio1,hochreiter}, accelerate optimization~\citep{andrychowicz2016learning}, and acquire priors suitable for few-shot learning~\citep{maml}. Modern meta-learning algorithms can broadly be classified into three high-level approaches: black-box meta-learners that parameterize a learning procedure using a neural network~\citep{mann,hugo,metanetworks,rl2,learningrl,mishra2017simple}, non-parametric meta-learners~\citep{siameseoneshot,matchingnets,snell2017prototypical}, and optimization-based meta-learners that embed an optimization procedure into the meta-learner~\citep{maml,metasgd,rusu2018meta,zintgraf2018fast,bertinetto2018meta,rajeswaran2019meta,lee2019meta,yoon2018bayesian,finn2018probabilistic}. We choose to build upon the latter class of optimization-based meta-learners, since they produce a well-formed optimization process that tends to be robust to out-of-distribution tasks, a useful characteristic in online meta-learning settings. 

While some works have evaluated meta-learning algorithms for $K$-shot $N$-way classification for a breadth of $K$ and $N$~\citep{snell2017prototypical,triantafillou2019meta,allen2019variadic,allen2019infinite,cactus,cao2020a}, these works typically train different networks for each value of $N$ and $K$, with some specifically noting poor generalization to values of $K$ not used in training~\citep{snell2017prototypical,cactus}. Unlike these works, we consider the setting where a single meta-learned model must handle multiple different values of $K$. This setting has been considered in black-box methods that receive datapoints and make predictions incrementally~\citep{mann,woodward2017active}, but this approach is known to underperform the setting where the model is trained for a specific value of $K$~\citep{mishra2017simple}. Recent works have proposed non-parametric meta-learners that work effectively with variable numbers of shots~\citep{allen2019variadic,cao2020a}. Non-parametric methods such as these prior works require at least one shot per class, whereas we consider a setting where there is even fewer datapoints available. This is possible in settings with non-mutually-exclusive tasks, such that the meta-learned model can provide a sufficiently strong prior about the class labels.

Our variable-shot meta-learning setting is specifically motivated by a problem setting that resembles online learning~\citep{ShaiBook} and continual learning~\citep{thrun1998lifelong}. It is well known that algorithms such as follow the leader (FTL) are computationally-expensive, and many works in online learning and continual learning focus on developing more computationally-efficient methods\rebuttal{~\citep{kirkpatrick2017overcoming,rebuffi2017icarl, li2017learning,gradient_episodic,forgetting, chaudhry2018efficient,zenke2017continual, tao2020few}}. Following multiple prior methods~\citep{ftml,lifelongreplay,rolnick2019experience}, we instead focus on settings where it is practical to maintain a replay buffer of data, and focus on the problem of effective forward transfer when presented data from a sequence of tasks. We do so by combining employing meta-learning in the online setting. Unlike prior online meta-learning works\rebuttal{~\citep{ftml,erin_openreview,khodak2019provable,zhuang2019online, ren2020wandering, antoniou2020defining, wallingford2020overfitting, yao2020online}}, we develop an algorithm that is specifically tailored to leverage variable amounts of data, allowing it to outperform a prior state-of-the-art online meta-learning approach~\citep{ftml}.
Finally, our work considers a problem setting that is distinct from works that a study online or continual learning in the \emph{inner loop} of meta-learning~\citep{AlShedivat2017ContinuousAV,nagabandi2018deep,javed2019meta,denevi2019online,he2019task,harrison2019continuous}.




%
